Regret, Delete, (Do Not) Repeat: An Analysis of Self-Cleaning Practices on Twitter After the Outbreak of the COVID-19 Pandemic

During the outbreak of the COVID-19 pandemic, many people shared their symptoms across Online Social Networks (OSNs) like Twitter, hoping for others' advice or moral support. Prior studies have shown that those who disclose health-related information across OSNs often tend to regret it and delete their publications afterwards. Hence, deleted posts containing sensitive data can be seen as manifestations of online regrets. In this work, we present an analysis of deleted content on Twitter during the outbreak of the COVID-19 pandemic. For this, we collected more than 3.67 million tweets describing COVID-19 symptoms (e.g., fever, cough, and fatigue) posted between January and April 2020. We observed that around 24% of the tweets containing personal pronouns were deleted either by their authors or by the platform after one year. As a practical application of the resulting dataset, we explored its suitability for the automatic classification of regrettable content on Twitter.

==> CHI LBW 2023 RegretCovid /review.tex <==
training_args = TrainingArguments(
    "deleted_tweets_trainer",                  # output folder
    evaluation_strategy='steps',      # used evaluate during the fine-tuning of our model
    learning_rate=2e-5,
    #per_device_train_batch_size=16 #we have checked with the size 16, 32 but it didn't work so default size is 8 
    )  

For BERT fine-tuning, we used pretrained distilbert-base-uncased model from huggingface\footnote{https://huggingface.co/distilbert-base-uncased}, the model for the tweets was trained for four epochs with a learning rate of 2e-5, with batch size of 16 with a sequence length of 128. 

For BERT fine-tuning, we used Huggin Face's pre-trained DistilBert base (uncased) with a learning rate of 2e-5, batch size 16, and a sequence length of 128.


max features?

maxlen? => used a batch size of 16 with a sequence length of 128




For TF-IDF we used Sklearn\footnote{https://scikit-learn.org/stable/modules/generated/sklearn.feature_extraction.text.TfidfTransformer.html} with its default configuration. 

from sklearn.feature_extraction.text import TfidfTransformer
preprocessing = Pipeline([
    ('vect', CountVectorizer()),
    ('tfidf', TfidfTransformer())
])
  




==> review.tex <==
training_args = TrainingArguments(
    "deleted_tweets_trainer",                  # output folder
    evaluation_strategy='steps',      # used evaluate during the fine-tuning of our model
    learning_rate=2e-5,
    #per_device_train_batch_size=16 #we have checked with the size 16, 32 but it didn't work so default size is 8 
    )  

For BERT fine-tuning, we used pretrained distilbert-base-uncased model from huggingface\footnote{https://huggingface.co/distilbert-base-uncased}, the model for the tweets was trained for four epochs with a learning rate of 2e-5, with batch size of 16 with a sequence length of 128. 

For BERT fine-tuning, we used Huggin Face's pre-trained DistilBert base (uncased) with a learning rate of 2e-5, batch size 16, and a sequence length of 128.


max features?

maxlen? => used a batch size of 16 with a sequence length of 128




For TF-IDF we used Sklearn\footnote{https://scikit-learn.org/stable/modules/generated/sklearn.feature_extraction.text.TfidfTransformer.html} with its default configuration. 

from sklearn.feature_extraction.text import TfidfTransformer
preprocessing = Pipeline([
    ('vect', CountVectorizer()),
    ('tfidf', TfidfTransformer())
])
  



